Sparse recovery of elliptic solvers from matrix-vector products

In this work, we show that solvers of elliptic boundary value problems in $d$ dimensions can be approximated to accuracy $\epsilon$ from only $\mathcal{O}\left(\log(N)\log^{d}(N / \epsilon)\right)$ matrix-vector products with carefully chosen vectors (right-hand sides). The solver is only accessed as a black box, and the underlying operator may be unknown and of an arbitrarily high order. Our algorithm (1) has complexity $\mathcal{O}\left(N\log^2(N)\log^{2d}(N / \epsilon)\right)$ and represents the solution operator as a sparse Cholesky factorization with $\mathcal{O}\left(N\log(N)\log^{d}(N / \epsilon)\right)$ nonzero entries, (2) allows for embarrassingly parallel evaluation of the solution operator and the computation of its log-determinant, (3) allows for $\mathcal{O}\left(\log(N)\log^{d}(N / \epsilon)\right)$ complexity computation of individual entries of the matrix representation of the solver that, in turn, enables its recompression to an $\mathcal{O}\left(N\log^{d}(N / \epsilon)\right)$ complexity representation. As a byproduct, our compression scheme produces a homogenized solution operator with near-optimal approximation accuracy. By polynomial approximation, we can also approximate the continuous Green's function (in operator and Hilbert-Schmidt norm) to accuracy $\epsilon$ from $\mathcal{O}\left(\log^{1 + d}\left(\epsilon^{-1}\right)\right)$ solutions of the PDE. We include rigorous proofs of these results. To the best of our knowledge, our algorithm achieves the best known trade-off between accuracy $\epsilon$ and the number of required matrix-vector products.

==> figures/tikz/matrix_heatmap.tex <==
\begin{axis}
    [
    view={90}{90},
    hide axis,
]

% \addplot3 [
%     mesh,
%     fill opacity=1.,
%     mesh/rows=16,
%     color=silver
% ] file {./figures/csv/decay_figure/decay_figure_q_4_zero_column.csv};
% %   \addplot table[x=a] {./figures/csv/decay_figure_q_L.csv};



\addplot3 [
    surf,
    mesh/rows=1024,
    colormap={CM}{color(-10)=(white) color(0)=(darkrust)},
%] file {./figures/csv/decay_figure/decay_figure_q_3_coordinate_L.csv};
] file {./figures/csv/decay_figure/decay_figure_q_5_coordinate_log10_L.csv};
%   \addplot table[x=a] {./figures/csv/decay_figure_q_L.csv};
    % \addplot table[x index={0}, y index={1}] {./figures/csv/decay_figure_q_3_L.csv};

\end{axis}

==> figures/tikz/matvec_plot.tex <==
\begin{axis}[
    axis lines = left,
    xlabel = \(\rho\),
    ylabel = \(\# \mathrm{matvecs}\),
    legend pos = north west,
    xmin = 3.5, xmax = 10.5,
    ymin = 0, ymax = 3000,
]
\addplot+[
    only marks,
    very thick,
    mark=+,
    color=rust,
    mark size=2.9pt]
table{./figures/csv/matvecs_vs_rho_q_6.csv};
\addlegendentry{\(N = 64^2\)}

\addplot+[
    only marks,
    very thick,
    mark=triangle,
    color=orange,
    mark size=2.9pt]
table{./figures/csv/matvecs_vs_rho_q_7.csv};
\addlegendentry{\(N = 128^2\)}

\addplot+[
    only marks,
    very thick,
    mark=square,
    color=lightblue,
    mark size=2.9pt]
table{./figures/csv/matvecs_vs_rho_q_8.csv};
\addlegendentry{\(N = 256^2\)}

\addplot+[
    only marks,
    very thick,
    color=seagreen,
    mark=o,
    mark size=2.9pt]
table{./figures/csv/matvecs_vs_rho_q_9.csv};
\addlegendentry{\(N = 512^2\)}
%Below the red parabola is defined
% \addplot [
%     domain=-10:10, 
%     samples=100, 
%     color=red,
% ]
% {x^2 - 2*x - 1};
% \addlegendentry{\(x^2 - 2x - 1\)}
% %Here the blue parabola is defined
% \addplot [
%     domain=-10:10, 
%     samples=100, 
%     color=blue,
%     ]
%     {x^2 + 2*x + 1};
% \addlegendentry{\(x^2 + 2x + 1\)}
% import the correct data from a CSV file
% \addplot table {figures/csv/n_threads_24_t_q_9_vary_rho.csv};
\end{axis}

==> figures/tikz/matvec_plot_dirichlet_mild_2d.tex <==
\begin{axis}[
    axis lines = left,
    xlabel = \(\rho\),
    ylabel = \(\# \mathrm{matvecs}\),
    legend pos = north west,
    xmin = 3.5, xmax = 10.5,
    ymin = 0, ymax = 4000,
]
\addplot+[
    only marks,
    very thick,
    mark=+,
    color=rust,
    mark size=2.9pt]
table[col sep=comma,x index=0,y index=1]{./figures/csv/rel_err_plots/poisson/64_2_dirichlet_constant_random_mild.csv};
\addlegendentry{\(N = 64^2\)}

\addplot+[
    only marks,
    very thick,
    mark=triangle,
    color=orange,
    mark size=2.9pt]
table[col sep=comma,x index=0,y index=1]{./figures/csv/rel_err_plots/poisson/128_2_dirichlet_constant_random_mild.csv};
\addlegendentry{\(N = 128^2\)}

\addplot+[
    only marks,
    very thick,
    mark=square,
    color=lightblue,
    mark size=2.9pt]
table[col sep=comma,x index=0,y index=1]{./figures/csv/rel_err_plots/poisson/256_2_dirichlet_constant_random_mild.csv};
\addlegendentry{\(N = 256^2\)}

\addplot+[
    only marks,
    very thick,
    color=seagreen,
    mark=o,
    mark size=2.9pt]
table[col sep=comma,x index=0,y index=1]{./figures/csv/rel_err_plots/poisson/512_2_dirichlet_constant_random_mild.csv};
\addlegendentry{\(N = 512^2\)}

\addplot+[
    only marks,
    very thick,
    color=joshua,
    mark=diamond,
    mark size=2.9pt]
table[col sep=comma,x index=0,y index=1]{./figures/csv/rel_err_plots/poisson/1024_2_dirichlet_constant_random_mild.csv};
\addlegendentry{\(N = 1024^2\)}


%Below the red parabola is defined
% \addplot [
%     domain=-10:10, 
%     samples=100, 
%     color=red,
% ]
% {x^2 - 2*x - 1};
% \addlegendentry{\(x^2 - 2x - 1\)}
% %Here the blue parabola is defined
% \addplot [
%     domain=-10:10, 
%     samples=100, 
%     color=blue,
%     ]
%     {x^2 + 2*x + 1};
% \addlegendentry{\(x^2 + 2x + 1\)}
% import the correct data from a CSV file
% \addplot table {figures/csv/n_threads_24_t_q_9_vary_rho.csv};
\end{axis}

==> figures/tikz/matvec_plot_neumann_mild_2d.tex <==
\begin{axis}[
    axis lines = left,
    xlabel = \(\rho\),
    ylabel = \(\# \mathrm{matvecs}\),
    legend pos = north west,
    xmin = 3.5, xmax = 10.5,
    ymin = 0, ymax = 4000,
]
\addplot+[
    only marks,
    very thick,
    mark=+,
    color=rust,
    mark size=2.9pt]
table[col sep=comma,x index=0,y index=1]{./figures/csv/rel_err_plots/poisson/64_2_neumann_constant_random_mild.csv};
\addlegendentry{\(N = 64^2\)}

\addplot+[
    only marks,
    very thick,
    mark=triangle,
    color=orange,
    mark size=2.9pt]
table[col sep=comma,x index=0,y index=1]{./figures/csv/rel_err_plots/poisson/128_2_neumann_constant_random_mild.csv};
\addlegendentry{\(N = 128^2\)}

\addplot+[
    only marks,
    very thick,
    mark=square,
    color=lightblue,
    mark size=2.9pt]
table[col sep=comma,x index=0,y index=1]{./figures/csv/rel_err_plots/poisson/256_2_neumann_constant_random_mild.csv};
\addlegendentry{\(N = 256^2\)}

\addplot+[
    only marks,
    very thick,
    color=seagreen,
    mark=o,
    mark size=2.9pt]
table[col sep=comma,x index=0,y index=1]{./figures/csv/rel_err_plots/poisson/512_2_neumann_constant_random_mild.csv};
\addlegendentry{\(N = 512^2\)}

\addplot+[
    only marks,
    very thick,
    color=joshua,
    mark=diamond,
    mark size=2.9pt]
table[col sep=comma,x index=0,y index=1]{./figures/csv/rel_err_plots/poisson/1024_2_neumann_constant_random_mild.csv};
\addlegendentry{\(N = 1024^2\)}


%Below the red parabola is defined
% \addplot [
%     domain=-10:10, 
%     samples=100, 
%     color=red,
% ]
% {x^2 - 2*x - 1};
% \addlegendentry{\(x^2 - 2x - 1\)}
% %Here the blue parabola is defined
% \addplot [
%     domain=-10:10, 
%     samples=100, 
%     color=blue,
%     ]
%     {x^2 + 2*x + 1};
% \addlegendentry{\(x^2 + 2x + 1\)}
% import the correct data from a CSV file
% \addplot table {figures/csv/n_threads_24_t_q_9_vary_rho.csv};
\end{axis}

==> figures/tikz/matvec_plot_periodic_severe_2d.tex <==
\begin{axis}[
    axis lines = left,
    xlabel = \(\rho\),
    ylabel = \(\# \mathrm{matvecs}\),
    legend pos = north west,
    xmin = 3.5, xmax = 10.5,
    ymin = 0, ymax = 4000,
]
\addplot+[
    only marks,
    very thick,
    mark=+,
    color=rust,
    mark size=2.9pt]
table[col sep=comma,x index=0,y index=1]{./figures/csv/rel_err_plots/poisson/64_2_periodic_random_severe_random_mild.csv};
\addlegendentry{\(N = 64^2\)}

\addplot+[
    only marks,
    very thick,
    mark=triangle,
    color=orange,
    mark size=2.9pt]
table[col sep=comma,x index=0,y index=1]{./figures/csv/rel_err_plots/poisson/128_2_periodic_random_severe_random_mild.csv};
\addlegendentry{\(N = 128^2\)}

\addplot+[
    only marks,
    very thick,
    mark=square,
    color=lightblue,
    mark size=2.9pt]
table[col sep=comma,x index=0,y index=1]{./figures/csv/rel_err_plots/poisson/256_2_periodic_random_severe_random_mild.csv};
\addlegendentry{\(N = 256^2\)}

\addplot+[
    only marks,
    very thick,
    color=seagreen,
    mark=o,
    mark size=2.9pt]
table[col sep=comma,x index=0,y index=1]{./figures/csv/rel_err_plots/poisson/512_2_periodic_random_severe_random_mild.csv};
\addlegendentry{\(N = 512^2\)}

\addplot+[
    only marks,
    very thick,
    color=joshua,
    mark=diamond,
    mark size=2.9pt]
table[col sep=comma,x index=0,y index=1]{./figures/csv/rel_err_plots/poisson/1024_2_periodic_random_severe_random_mild.csv};
\addlegendentry{\(N = 1024^2\)}


%Below the red parabola is defined
% \addplot [
%     domain=-10:10, 
%     samples=100, 
%     color=red,
% ]
% {x^2 - 2*x - 1};
% \addlegendentry{\(x^2 - 2x - 1\)}
% %Here the blue parabola is defined
% \addplot [
%     domain=-10:10, 
%     samples=100, 
%     color=blue,
%     ]
%     {x^2 + 2*x + 1};
% \addlegendentry{\(x^2 + 2x + 1\)}
% import the correct data from a CSV file
% \addplot table {figures/csv/n_threads_24_t_q_9_vary_rho.csv};
\end{axis}

==> figures/tikz/rel_err_plot.tex <==
\begin{semilogyaxis}[
    axis lines = left,
    xlabel = \(\rho\),
    ylabel = \(\|\KM - \dL \dL^{\top}\| / \|\KM\|\),
    legend pos = north east,
    xmin = 3.5, xmax = 10.5,
]
\addplot+[
    only marks,
    very thick,
    mark=+,
    color=rust,
    mark size=2.9pt]
table{./figures/csv/err_vs_rho_q_6.csv};
\addlegendentry{\(N = 64^2\)}

\addplot+[
    only marks,
    very thick,
    mark=triangle,
    color=orange,
    mark size=2.9pt]
table{./figures/csv/err_vs_rho_q_7.csv};
\addlegendentry{\(N = 128^2\)}

\addplot+[
    only marks,
    very thick,
    mark=square,
    color=lightblue,
    mark size=2.9pt]
table{./figures/csv/err_vs_rho_q_8.csv};
\addlegendentry{\(N = 256^2\)}

\addplot+[
    only marks,
    very thick,
    color=seagreen,
    mark=o,
    mark size=2.9pt]
table{./figures/csv/err_vs_rho_q_9.csv};
\addlegendentry{\(N = 512^2\)}
%Below the red parabola is defined
% \addplot [
%     domain=-10:10, 
%     samples=100, 
%     color=red,
% ]
% {x^2 - 2*x - 1};
% \addlegendentry{\(x^2 - 2x - 1\)}
% %Here the blue parabola is defined
% \addplot [
%     domain=-10:10, 
%     samples=100, 
%     color=blue,
%     ]
%     {x^2 + 2*x + 1};
% \addlegendentry{\(x^2 + 2x + 1\)}
% import the correct data from a CSV file
% \addplot table {figures/csv/n_threads_24_t_q_9_vary_rho.csv};
\end{semilogyaxis}

==> figures/tikz/rel_err_plot_dirichlet_mild_2d.tex <==
\begin{semilogyaxis}[
    axis lines = left,
    xlabel = \(\rho\),
    ylabel = \(\|\KM - \dL \dL^{\top}\| / \|\KM\|\),
    legend pos = north east,
    xmin = 3.5, xmax = 10.5,
]
\addplot+[
    only marks,
    very thick,
    mark=+,
    color=rust,
    mark size=2.9pt]
table[col sep=comma,x index=0,y index=2]{./figures/csv/rel_err_plots/poisson/64_2_dirichlet_constant_random_mild.csv};
\addlegendentry{\(N = 64^2\)}

\addplot+[
    only marks,
    very thick,
    mark=triangle,
    color=orange,
    mark size=2.9pt]
table[col sep=comma,x index=0,y index=2]{./figures/csv/rel_err_plots/poisson/128_2_dirichlet_constant_random_mild.csv};
\addlegendentry{\(N = 128^2\)}

\addplot+[
    only marks,
    very thick,
    mark=square,
    color=lightblue,
    mark size=2.9pt]
table[col sep=comma,x index=0,y index=2]{./figures/csv/rel_err_plots/poisson/256_2_dirichlet_constant_random_mild.csv};
\addlegendentry{\(N = 256^2\)}

\addplot+[
    only marks,
    very thick,
    color=seagreen,
    mark=o,
    mark size=2.9pt]
    table[col sep=comma,x index=0,y index=2]{./figures/csv/rel_err_plots/poisson/512_2_dirichlet_constant_random_mild.csv};
\addlegendentry{\(N = 512^2\)}

\addplot+[
    only marks,
    very thick,
    color=joshua,
    mark=diamond,
    mark size=2.9pt]
    table[col sep=comma,x index=0,y index=2]{./figures/csv/rel_err_plots/poisson/512_2_dirichlet_constant_random_mild.csv};
\addlegendentry{\(N = 1024^2\)}

%Below the red parabola is defined
% \addplot [
%     domain=-10:10, 
%     samples=100, 
%     color=red,
% ]
% {x^2 - 2*x - 1};
% \addlegendentry{\(x^2 - 2x - 1\)}
% %Here the blue parabola is defined
% \addplot [
%     domain=-10:10, 
%     samples=100, 
%     color=blue,
%     ]
%     {x^2 + 2*x + 1};
% \addlegendentry{\(x^2 + 2x + 1\)}
% import the correct data from a CSV file
% \addplot table {figures/csv/n_threads_24_t_q_9_vary_rho.csv};
\end{semilogyaxis}

==> figures/tikz/rel_err_plot_dirichlet_mild_3d.tex <==
\begin{semilogyaxis}[
    axis lines = left,
    xlabel = \(\rho\),
    ylabel = \(\|\KM - \dL \dL^{\top}\| / \|\KM\|\),
    legend pos = north east,
    xmin = 2.5, xmax = 6.5,
]
\addplot+[
    only marks,
    very thick,
    mark=x,
    color=silver,
    mark size=2.9pt]
table[col sep=comma,x index=0,y index=2]{./figures/csv/rel_err_plots/poisson/32_3_dirichlet_constant_random_mild.csv};
\addlegendentry{\(N = 32^3\)}


\addplot+[
    only marks,
    very thick,
    mark=+,
    color=rust,
    mark size=2.9pt]
table[col sep=comma,x index=0,y index=2]{./figures/csv/rel_err_plots/poisson/64_3_dirichlet_constant_random_mild.csv};
\addlegendentry{\(N = 64^3\)}

% \addplot+[
%     only marks,
%     very thick,
%     mark=triangle,
%     color=orange,
%     mark size=2.9pt]
% table[col sep=comma,x index=0,y index=2]{./figures/csv/rel_err_plots/poisson/128_2_dirichlet_constant_random_mild.csv};
% \addlegendentry{\(N = 128^2\)}



%Below the red parabola is defined
% \addplot [
%     domain=-10:10, 
%     samples=100, 
%     color=red,
% ]
% {x^2 - 2*x - 1};
% \addlegendentry{\(x^2 - 2x - 1\)}
% %Here the blue parabola is defined
% \addplot [
%     domain=-10:10, 
%     samples=100, 
%     color=blue,
%     ]
%     {x^2 + 2*x + 1};
% \addlegendentry{\(x^2 + 2x + 1\)}
% import the correct data from a CSV file
% \addplot table {figures/csv/n_threads_24_t_q_9_vary_rho.csv};
\end{semilogyaxis}

==> figures/tikz/rel_err_plot_neumann_mild_2d.tex <==
\begin{semilogyaxis}[
    axis lines = left,
    xlabel = \(\rho\),
    ylabel = \(\|\KM - \dL \dL^{\top}\| / \|\KM\|\),
    legend pos = north east,
    xmin = 3.5, xmax = 10.5,
]
\addplot+[
    only marks,
    very thick,
    mark=+,
    color=rust,
    mark size=2.9pt]
table[col sep=comma,x index=0,y index=2]{./figures/csv/rel_err_plots/poisson/64_2_neumann_constant_random_mild.csv};
\addlegendentry{\(N = 64^2\)}

\addplot+[
    only marks,
    very thick,
    mark=triangle,
    color=orange,
    mark size=2.9pt]
table[col sep=comma,x index=0,y index=2]{./figures/csv/rel_err_plots/poisson/128_2_neumann_constant_random_mild.csv};
\addlegendentry{\(N = 128^2\)}

\addplot+[
    only marks,
    very thick,
    mark=square,
    color=lightblue,
    mark size=2.9pt]
table[col sep=comma,x index=0,y index=2]{./figures/csv/rel_err_plots/poisson/256_2_neumann_constant_random_mild.csv};
\addlegendentry{\(N = 256^2\)}

\addplot+[
    only marks,
    very thick,
    color=seagreen,
    mark=o,
    mark size=2.9pt]
    table[col sep=comma,x index=0,y index=2]{./figures/csv/rel_err_plots/poisson/512_2_neumann_constant_random_mild.csv};
\addlegendentry{\(N = 512^2\)}

\addplot+[
    only marks,
    very thick,
    color=joshua,
    mark=diamond,
    mark size=2.9pt]
    table[col sep=comma,x index=0,y index=2]{./figures/csv/rel_err_plots/poisson/512_2_neumann_constant_random_mild.csv};
\addlegendentry{\(N = 1024^2\)}

%Below the red parabola is defined
% \addplot [
%     domain=-10:10, 
%     samples=100, 
%     color=red,
% ]
% {x^2 - 2*x - 1};
% \addlegendentry{\(x^2 - 2x - 1\)}
% %Here the blue parabola is defined
% \addplot [
%     domain=-10:10, 
%     samples=100, 
%     color=blue,
%     ]
%     {x^2 + 2*x + 1};
% \addlegendentry{\(x^2 + 2x + 1\)}
% import the correct data from a CSV file
% \addplot table {figures/csv/n_threads_24_t_q_9_vary_rho.csv};
\end{semilogyaxis}
